Example Setups of Navier-Stokes Equations with Control and Observation: Spatial Discretization and Representation via Linear-quadratic Matrix Coefficients

We provide spatial discretizations of nonlinear incompressible Navier-Stokes equations with inputs and outputs in the form of matrices ready to use in any numerical linear algebra package. We discuss the assembling of the system operators and the realization of boundary conditions and inputs and outputs. We describe the two benchmark problems - the driven cavity and the cylinder wake - and provide the corresponding data. The use of the data is illustrated by numerous example setups. The test cases are provided as plain PYTHON or OCTAVE/MATLAB script files for immediate replication.

==> discnrefs.tex <==
\section{Discussion}\label{sec:discnrefs}

The provided data is to be used to test control and model reduction techniques in generic Navier-Stokes setups.

For a numerical analysis of the problem the following issues have to be considered
\begin{itemize}
	\item existence of solutions 
	\item suitability of the boundary conditions
	\item other approaches to boundary control (Raymond, Weichelt, weak)
	\item modelling of the input operator
	\item controllability and observability or stabilizability and detectability
	\item consistency of the spatial discretization
\end{itemize}

